Do Discrete Self-Supervised Representations of Speech Capture Tone Distinctions?

Discrete representations of speech, obtained from Self-Supervised Learning (SSL) foundation models, are widely used, especially where there are limited data for the downstream task, such as for a low-resource language. Typically, discretization of speech into a sequence of symbols is achieved by unsupervised clustering of the latents from an SSL model. Our study evaluates whether discrete symbols - found using k-means - adequately capture tone in two example languages, Mandarin and Yoruba. We compare latent vectors with discrete symbols, obtained from HuBERT base, MandarinHuBERT, or XLS-R, for vowel and tone classification. We find that using discrete symbols leads to a substantial loss of tone information, even for language-specialised SSL models. We suggest that discretization needs to be task-aware, particularly for tone-dependent downstream tasks.

==> correlation_plot2.tex <==
\begin{figure*}[h!]
  \centering
  \hspace{0.01cm} % Virtually no space on the left
  \begin{subfigure}{0.9\textwidth} % Adjust width to avoid overflow
    \includegraphics[width=0.9\linewidth]{corr_plot/trial2.pdf}
    \caption{Yoruba on HuBERT base and Yoruba on XLS-R}
    \label{fig:yoruba_vowels}
  \end{subfigure}
  \hspace{1cm} % Add space on the right
\end{figure*}
